Crafting Desirable Climate Trajectories with RL Explored Socio-Environmental Simulations

Climate change poses an existential threat, necessitating effective climate policies to enact impactful change. Decisions in this domain are incredibly complex, involving conflicting entities and evidence. In the last decades, policymakers increasingly use simulations and computational methods to guide some of their decisions. Integrated Assessment Models (IAMs) are one of such methods, which combine social, economic, and environmental simulations to forecast potential policy effects. For example, the UN uses outputs of IAMs for their recent Intergovernmental Panel on Climate Change (IPCC) reports. Traditionally these have been solved using recursive equation solvers, but have several shortcomings, e.g. struggling at decision making under uncertainty. Recent preliminary work using Reinforcement Learning (RL) to replace the traditional solvers shows promising results in decision making in uncertain and noisy scenarios. We extend on this work by introducing multiple interacting RL agents as a preliminary analysis on modelling the complex interplay of socio-interactions between various stakeholders or nations that drives much of the current climate crisis. Our findings show that cooperative agents in this framework can consistently chart pathways towards more desirable futures in terms of reduced carbon emissions and improved economy. However, upon introducing competition between agents, for instance by using opposing reward functions, desirable climate futures are rarely reached. Modelling competition is key to increased realism in these simulations, as such we employ policy interpretation by visualising what states lead to more uncertain behaviour, to understand algorithm failure. Finally, we highlight the current limitations and avenues for further work to ensure future technology uptake for policy derivation.

==> images_for_critical_states.tex <==
2_agents
new_rnn_comp_tests_1713785448397_...
PBPB
10

PBmaxA
5

PBmaxY
6(succeed),9(notsucceed)


3_agents - issues here are that it does not have the correct ending cus I cut the thing lol so will have to find a previous runs one so instead gonna use the :
new_rnn_comp_tests_1713785465938

PBPBPB
6,12 

PBPBmaxY
8

PBPBmaxA
10

PBmaxAmaxA
9

PBmaxYmaxY
13

PBmaxAmaxY
11

maybe 21 good for the other thing
